Parallel and Proximal Constrained Linear-Quadratic Methods for Real-Time Nonlinear MPC

Recent strides in nonlinear model predictive control (NMPC) underscore a dependence on numerical advancements to efficiently and accurately solve large-scale problems. Given the substantial number of variables characterizing typical whole-body optimal control (OC) problems - often numbering in the thousands - exploiting the sparse structure of the numerical problem becomes crucial to meet computational demands, typically in the range of a few milliseconds. Addressing the linear-quadratic regulator (LQR) problem is a fundamental building block for computing Newton or Sequential Quadratic Programming (SQP) steps in direct optimal control methods. This paper concentrates on equality-constrained problems featuring implicit system dynamics and dual regularization, a characteristic of advanced interiorpoint or augmented Lagrangian solvers. Here, we introduce a parallel algorithm for solving an LQR problem with dual regularization. Leveraging a rewriting of the LQR recursion through block elimination, we first enhanced the efficiency of the serial algorithm and then subsequently generalized it to handle parametric problems. This extension enables us to split decision variables and solve multiple subproblems concurrently. Our algorithm is implemented in our nonlinear numerical optimal control library ALIGATOR. It showcases improved performance over previous serial formulations and we validate its efficacy by deploying it in the model predictive control of a real quadruped robot.

==> Makefile <==
FILE = main.tex

default:
	latexmk -pdf $(FILE)

diff:
	mkdir -p tmpdiff
	git latexdiff --type=CFONT --view --latexmk \
		--config="PICTUREENV=(?:picture|DIFnomarkup|tabular)[\w\d*@]*" \
		--tmpdirprefix tmpdiff --main $(FILE) --run-biber \
		submission -- -o diff.pdf

